Rapid wavefront shaping using an optical gradient acquisition

Wavefront shaping systems aim to image deep into scattering tissue by reshaping incoming and outgoing light to correct aberrations caused by tissue inhomogeneity However, the desired modulation depends on the unknown tissue structure and therefore its estimation is a challenging time-consuming task. Most strategies rely on coordinate descent optimization, which sequentially varies each modulation parameter and assesses its impact on the resulting image. We propose a rapid wavefront shaping scheme that transitions from coordinate descent to gradient descent optimization, using the same measurement to update all modulation parameters simultaneously. To achieve this, we have developed an analytical framework that expresses the gradient of the wavefront shaping score with respect to all modulation parameters. Although this gradient depends on the unknown tissue structure, we demonstrate how it can be inferred from the optical system's measurements. Our new framework enables rapid inference of wavefront shaping modulations. Additionally, since the complexity of our algorithm does not scale with the number of modulation parameters, we can achieve very high-resolution modulations, leading to better corrections in thicker tissue layers. We showcase the effectiveness of our framework in correcting aberrations in a coherent confocal microscope.

==> abstract.tex <==
\begin{abstract}


A fundamental limitation of spatial light modulation (SLM) devices is that their \etnd, defined as the product of the display's size and angular range, is bounded by the number of pixel units. 
%%
Current SLMs are woefully inadequate in meeting the spatial and angular ranges of many real applications. In particular using these SLMs to generate realistic computer-controlled holographic displays  would require scaling the number of display units by a few orders of magnitude.
%%
%
%
In this work, we suggest that rather than excessively increasing the pixel count, \etnd can be expanded by augmenting the display units with tilting capabilities. 
%
Furthermore, we show that tiltable displays can be realized using a cascade of binary tilt layers, each capable of tilting the light towards one of two orientations. With proper design, the \etnd-expansion factor scales {\em exponentially} with the  number of display layers; hence, a very small number of such layers can effectively realize wide expansion factors.
%
We implement a proof of concept  display and demonstrate its applicability for displaying multi-view or holographic content with increased size and angular field-of-view.



%This paper proposes a class of \etnd-expansion designs using the family of piecewise linear phase modulations, which can tilt the display output into a larger range of directions.
%We realize  a restricted form of a tiltable display   using a novel lab prototype.


\end{abstract}

==> fig_beads.tex <==
\begin{figure*}[t!]
	\begin{center}		
		\begin{tabular}{@{}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}}			
			\multicolumn{4}{c}{\hspace{-0.6cm}\large One point }& 
			\multicolumn{2}{c}{\hspace{-0.6cm}\large Confocal scan}&
			\multicolumn{1}{c}{\hspace{-0.6cm}\large Wide field}\\
			\multicolumn{2}{c}{\hspace{-0.6cm} Main cam.} & 
			\multicolumn{2}{c}{\hspace{-0.6cm} Valid. cam.} & 
			\multicolumn{2}{c}{\hspace{-0.6cm} Main cam.} & 
			\multicolumn{1}{c}{\hspace{-0.6cm} Valid. cam.} \\
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize w/o}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize w/ }&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize w/o}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize w/ }&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize w/o}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize w/ }&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize Incoherent}\\
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize modulation}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize modulation}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize modulation}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize modulation}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize modulation}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize modulation}&	
			\multicolumn{1}{c}{\hspace{-0.6cm} \scriptsize illumination}\\
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/maininit_bead1.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/mainfinal_bead1.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/validinit_bead1.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/validfinal_bead1.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/Iinit_bead1.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/Ifinal_bead1.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead1/ref_bead1.png}\\
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/maininit_bead2.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/mainfinal_bead2.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/validinit_bead2.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/validfinal_bead2.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/Iinit_bead2.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/Ifinal_bead2.png}&
			\includegraphics[width= 0.14\textwidth]{figs/beads/bead2/ref_bead2.png}
		\end{tabular}
		\caption{\textbf{Confcal scan of beads:} We show that our algorithm can also be applied on sparser targets. We dispersed $3\um$ polystyrene beads in agarose gel and image them. Columns 1-2: Main camera images of a single focal spot before and after optimization. Columns 3-4: Corresponding validation camera images. Columns 5-7: Confocal scanning results: Without aberration correction, with aberration correction, and reference image of the target captured by illuminating the sample with incoherent light and capturing with the validation camera.}
		\label{fig:beads}
	\end{center}
\end{figure*}


==> fig_multiconj_setup.tex <==
\begin{figure*}[t!]
	\begin{center}
		\includegraphics[width= 0.85\textwidth]{figs/setup/multiconj.pdf}
	\end{center}
	\caption{{\bf{Setup for multi-conjugate confocal correction:}} An incoming laser beam is directed to focus on a point inside the tissue, the focal point can be shifted with a galvo. The figure illustrates two such tilted paths in two shades of green. On its way to the sample the beam passes through a relay system,  containing an SLM for aberration correction. The SLM is placed such that it is conjugate to a  plane inside the tissue volume.  The emitted light is returning via the same path and collected by a point detector (or a single pixel on a 2D sensor). After the dichrioc mirror there is an additional SLM used to implement the interferometer.  }\label{fig:setup_multiconj}
\end{figure*}



==> fig_onion_no_scatter.tex <==
\begin{figure*}[t!]
	\begin{center}		
		\begin{tabular}{@{}c@{~~~~~~~~}c@{~}}			
			\multicolumn{2}{c}{\hspace{0cm}\huge No scatter }\\ 
			\multicolumn{1}{c}{\hspace{-1cm}\large Valid. Cam.}& 
			\multicolumn{1}{c}{\hspace{0cm}\large Main Cam. }\\
			\multicolumn{1}{c}{\hspace{-1cm}\large Incoherent illumination }& 
			\multicolumn{1}{c}{\hspace{0cm} \large Confocal Scan}\\
			\includegraphics[width= 0.30\textwidth]{figs/onion/ref_incoherent.png}&
			\includegraphics[width= 0.30\textwidth]{figs/onion/ref_confocal.png}\\
		\end{tabular}
		\caption{\textbf{Onion cells without scattering:} \blue{We present a confocal scan of a thin onion cells without much scattering. The onion cells here are different than the ones presented in the main text; however, they visualize similar structure, the cell are bright and the boundaries are darker. }}
		\label{fig:onion_no_scatter_sup}
	\end{center}
\end{figure*}

